AdapterTune: Zero-Initialized Low-Rank Adapters for Frozen Vision Transformers

Frozen-backbone transfer with Vision Transformers faces two under-addressed issues: optimization instability when adapters are naively inserted into a fixed feature extractor, and the absence of principled guidance for setting adapter capacity. We introduce AdapterTune, which augments each transformer block with a residual low-rank bottleneck whose up-projection is zero-initialized, guaranteeing that the adapted network starts exactly at the pretrained function and eliminates early-epoch representation drift. On the analytical side, we formalize adapter rank as a capacity budget for approximating downstream task shifts in feature space. The resulting excess-risk decomposition predicts monotonic but diminishing accuracy gains with increasing rank, an ``elbow'' behavior we confirm through controlled sweeps. We evaluate on 9 datasets and 3 backbone scales with multi-seed reporting throughout. On a core 5 dataset transfer suite, AdapterTune improves top-1 accuracy over head-only transfer by +14.9 points on average while training only 0.92 of the parameters required by full fine-tuning, and outperforms full fine-tuning on 10 of 15 dataset-backbone pairs. Across the full benchmark, AdapterTune improves over head-only transfer on every dataset-backbone pair tested. Ablations on rank, placement, and initialization isolate each design choice. The code is available at: https://github.com/salimkhazem/adaptertune

==> tables/all_benchmarks_results.tex <==
% Auto-generated extended benchmark results table — do not edit directly
% Format: mean ± std over deduplicated seed runs; bold = best method per dataset/backbone
\begin{tabular}{llccc}
\toprule
\multirow{2}{*}{Dataset} & \multirow{2}{*}{Backbone}
  & Head-Only & \method (Ours) & Full FT \\
  & & Top-1 (\%) & Top-1 (\%) & Top-1 (\%) \\
\midrule
  \multirow{3}{*}{CIFAR-10} & ViT-S/16 & $89.71_{\pm0.04}$ & $\mathbf{97.48}_{\pm0.05}$ & $97.20_{\pm0.00}$ \\
   & ViT-B/16 & $94.76_{\pm0.04}$ & $\mathbf{98.86}_{\pm0.04}$ & $95.28_{\pm0.16}$ \\
   & DeiT-T & $87.66_{\pm0.11}$ & $95.54_{\pm0.11}$ & $\mathbf{96.74}_{\pm0.01}$ \\
\midrule
  \multirow{3}{*}{CIFAR-100} & ViT-S/16 & $71.99_{\pm0.28}$ & $\mathbf{84.88}_{\pm0.06}$ & $79.57_{\pm0.11}$ \\
   & ViT-B/16 & $81.53_{\pm0.23}$ & $\mathbf{91.21}_{\pm0.10}$ & $80.65_{\pm1.84}$ \\
   & DeiT-T & $68.00_{\pm0.56}$ & $\mathbf{80.32}_{\pm0.10}$ & $79.73_{\pm0.25}$ \\
\midrule
  \multirow{3}{*}{SVHN} & ViT-S/16 & $54.46_{\pm0.04}$ & $96.18_{\pm0.09}$ & $\mathbf{97.35}_{\pm0.01}$ \\
   & ViT-B/16 & $65.45_{\pm0.61}$ & $\mathbf{97.47}_{\pm0.06}$ & $97.47_{\pm0.02}$ \\
   & DeiT-T & $44.48_{\pm0.90}$ & $95.32_{\pm0.10}$ & $\mathbf{97.21}_{\pm0.01}$ \\
\midrule
  \multirow{3}{*}{Oxford-IIIT Pet} & ViT-S/16 & $90.46_{\pm0.12}$ & $\mathbf{93.46}_{\pm0.06}$ & $89.51_{\pm0.04}$ \\
   & ViT-B/16 & $93.30_{\pm0.28}$ & $\mathbf{94.27}_{\pm0.17}$ & $86.62_{\pm1.12}$ \\
   & DeiT-T & $90.77_{\pm0.24}$ & $\mathbf{91.41}_{\pm0.03}$ & $88.99_{\pm0.29}$ \\
\midrule
  \multirow{3}{*}{Food101} & ViT-S/16 & $68.78_{\pm0.07}$ & $85.02_{\pm0.02}$ & $\mathbf{86.46}_{\pm0.07}$ \\
   & ViT-B/16 & $84.32_{\pm0.05}$ & $\mathbf{90.90}_{\pm0.10}$ & $84.41_{\pm0.31}$ \\
   & DeiT-T & $66.01_{\pm0.08}$ & $80.55_{\pm0.07}$ & $\mathbf{85.10}_{\pm0.15}$ \\
\midrule
  \multirow{3}{*}{Flowers102} & ViT-S/16 & $87.73_{\pm0.53}$ & $\mathbf{94.43}_{\pm0.04}$ & $92.92_{\pm0.73}$ \\
   & ViT-B/16 & $98.71_{\pm0.11}$ & $\mathbf{99.43}_{\pm0.04}$ & $93.23_{\pm2.75}$ \\
   & DeiT-T & $85.87_{\pm0.21}$ & $\mathbf{94.19}_{\pm0.11}$ & $93.18_{\pm0.18}$ \\
\midrule
  \multirow{3}{*}{ImageNet-R} & ViT-S/16 & $46.94_{\pm0.66}$ & $\mathbf{69.26}_{\pm0.41}$ & $59.59_{\pm0.28}$ \\
   & ViT-B/16 & $62.17_{\pm0.66}$ & $\mathbf{80.10}_{\pm0.41}$ & $57.66_{\pm0.22}$ \\
   & DeiT-T & $49.41_{\pm0.85}$ & $\mathbf{65.22}_{\pm0.22}$ & $59.06_{\pm0.32}$ \\
\midrule
  \multirow{3}{*}{Tiny-ImageNet} & ViT-S/16 & $73.69_{\pm0.12}$ & $\mathbf{84.95}_{\pm0.07}$ & $71.38_{\pm0.97}$ \\
   & ViT-B/16 & $81.45_{\pm0.09}$ & $\mathbf{90.00}_{\pm0.09}$ & $71.99_{\pm2.73}$ \\
   & DeiT-T & $70.28_{\pm0.18}$ & $\mathbf{76.35}_{\pm0.15}$ & $69.04_{\pm0.37}$ \\
\midrule
  \multirow{3}{*}{FGVC-Aircraft} & ViT-S/16 & $36.70_{\pm0.22}$ & $67.72_{\pm0.22}$ & $\mathbf{68.28}_{\pm0.79}$ \\
   & ViT-B/16 & $52.14_{\pm0.09}$ & $\mathbf{74.79}_{\pm0.78}$ & $69.86_{\pm1.14}$ \\
   & DeiT-T & $37.56_{\pm0.51}$ & $65.73_{\pm0.26}$ & $\mathbf{72.51}_{\pm0.73}$ \\
\bottomrule
\end{tabular}


==> tables/hparam_sensitivity_cifar10_vitsmall.tex <==
% Auto-generated hyperparameter sensitivity table — do not edit directly
% CIFAR-10 / ViT-S/16 adapter ablations (rank=16, every=1, zero init)
\begin{tabular}{llcc}
\toprule
Axis & Setting & Top-1 (\%) & $\Delta$ \\
\midrule
  \multirow{3}{*}{LR} & $2.5\times 10^{-4}$ & $97.56_{\pm0.10}$ & -0.12 \\
   & $5\times 10^{-4}$ & $\mathbf{97.68}_{\pm0.07}$ & +0.00 \\
   & $10^{-3}$ & $97.61_{\pm0.02}$ & -0.08 \\
\midrule
  \multirow{3}{*}{WD} & 0.01 & $97.54_{\pm0.07}$ & -0.07 \\
   & 0.05 & $97.61_{\pm0.02}$ & +0.00 \\
   & 0.1 & $\mathbf{97.79}_{\pm0.06}$ & +0.18 \\
\midrule
  \multirow{3}{*}{$\alpha$} & 0.5 & $\mathbf{97.70}_{\pm0.05}$ & +0.09 \\
   & 1 & $97.61_{\pm0.02}$ & +0.00 \\
   & 2 & $97.47_{\pm0.08}$ & -0.14 \\
\bottomrule
\end{tabular}


==> tables/table_ablation_rank.tex <==
\begin{table}[t]
\centering
\caption{Ablation: effect of adapter rank $r$ on Top-1 test accuracy (mean\,±\,std, 3 seeds).}
\label{tab:ablation_rank}
\setlength{\tabcolsep}{4pt}
\footnotesize
\begin{tabular}{l l r r}
\toprule
\textbf{Backbone} & \textbf{Rank $r$} & \textbf{CIFAR-10} & \textbf{CIFAR-100} \\
\midrule
\multirow{4}{*}{DeiT-Ti/16}
  & $r=8$ & 95.98\,±\,0.08 & 80.63\,±\,0.23 \\
  & $r=16$ & 96.44\,±\,0.04 & 81.47\,±\,0.27 \\
  & $r=32$ & 96.63\,±\,0.03 & 81.66\,±\,0.23 \\
  & $r=64$ & 96.87\,±\,0.21 & 82.19\,±\,0.16 \\
\midrule
\multirow{4}{*}{ViT-S/16}
  & $r=8$ & 97.56\,±\,0.14 & 85.15\,±\,0.06 \\
  & $r=16$ & 97.61\,±\,0.02 & 85.07\,±\,0.23 \\
  & $r=32$ & 97.75\,±\,0.06 & 85.22\,±\,0.00 \\
  & $r=64$ & 97.85\,±\,0.11 & 85.13\,±\,0.00 \\
\midrule
\multirow{4}{*}{ViT-B/16}
  & $r=8$ & 98.89\,±\,0.00 & 91.11\,±\,0.00 \\
  & $r=16$ & 99.11\,±\,0.00 & 91.15\,±\,0.00 \\
  & $r=32$ & 98.86\,±\,0.00 & 91.56\,±\,0.00 \\
  & $r=64$ & 98.97\,±\,0.00 & 91.06\,±\,0.00 \\
\midrule
\bottomrule
\end{tabular}
\end{table}

==> tables/table_main_results.tex <==
\begin{table}[t]
\centering
\caption{Top-1 test accuracy (\%) on all benchmarks (mean\,±\,std over 3 seeds). \textbf{Bold}: best per column. AdaptTuner uses rank $r=16$, every block, zero-init.}
\label{tab:main_results}
\setlength{\tabcolsep}{4pt}
\footnotesize
\begin{tabular}{l l r r r r r r r r r}
\toprule
\textbf{Backbone} & \textbf{Method} & \textbf{CIFAR-10} & \textbf{CIFAR-100} & \textbf{SVHN} & \textbf{Oxford Pets} & \textbf{Food-101} & \textbf{Flowers-102} & \textbf{FGVC-Aircraft} & \textbf{ImageNet-R} & \textbf{Tiny-ImageNet} \\
\midrule
\multirow{3}{*}{DeiT-Ti/16}
  & Head-Only & 87.66\,±\,0.13 & 68.00\,±\,0.68 & 44.48\,±\,1.10 & 90.77\,±\,0.29 & 66.01\,±\,0.09 & 85.87\,±\,0.26 & 37.56\,±\,0.62 & 49.41\,±\,1.04 & 70.28\,±\,0.23 \\
  & Full Fine-Tune & \textbf{96.74\,±\,0.02} & 79.73\,±\,0.31 & \textbf{97.21\,±\,0.01} & 88.99\,±\,0.35 & \textbf{85.10\,±\,0.18} & 93.18\,±\,0.22 & \textbf{72.51\,±\,0.90} & 59.06\,±\,0.39 & 69.04\,±\,0.46 \\
  & \textbf{AdaptTuner (Ours)} & 95.54\,±\,0.13 & \textbf{80.32\,±\,0.13} & 95.32\,±\,0.12 & \textbf{91.41\,±\,0.04} & 80.55\,±\,0.08 & \textbf{94.19\,±\,0.13} & 65.73\,±\,0.32 & \textbf{65.22\,±\,0.27} & \textbf{76.35\,±\,0.18} \\
\midrule
\multirow{3}{*}{ViT-S/16}
  & Head-Only & 89.71\,±\,0.04 & 71.99\,±\,0.34 & 54.46\,±\,0.05 & 90.46\,±\,0.14 & 68.78\,±\,0.08 & 87.73\,±\,0.64 & 36.70\,±\,0.27 & 46.94\,±\,0.81 & 73.69\,±\,0.14 \\
  & Full Fine-Tune & 97.20\,±\,0.01 & 79.57\,±\,0.14 & \textbf{97.35\,±\,0.02} & 89.51\,±\,0.05 & \textbf{86.46\,±\,0.08} & 92.92\,±\,0.89 & \textbf{68.28\,±\,0.96} & 59.59\,±\,0.34 & 71.38\,±\,1.18 \\
  & \textbf{AdaptTuner (Ours)} & \textbf{97.48\,±\,0.06} & \textbf{84.88\,±\,0.08} & 96.18\,±\,0.11 & \textbf{93.46\,±\,0.07} & 85.02\,±\,0.03 & \textbf{94.43\,±\,0.05} & 67.72\,±\,0.27 & \textbf{69.26\,±\,0.50} & \textbf{84.95\,±\,0.09} \\
\midrule
\multirow{3}{*}{ViT-B/16}
  & Head-Only & 94.76\,±\,0.05 & 81.53\,±\,0.28 & 65.45\,±\,0.74 & 93.30\,±\,0.34 & 84.32\,±\,0.06 & 98.71\,±\,0.14 & 52.14\,±\,0.11 & 62.17\,±\,0.81 & 81.45\,±\,0.11 \\
  & Full Fine-Tune & 95.28\,±\,0.20 & 80.65\,±\,2.25 & \textbf{97.47\,±\,0.02} & 86.62\,±\,1.37 & 84.41\,±\,0.38 & 93.23\,±\,3.37 & 69.86\,±\,1.40 & 57.66\,±\,0.27 & 71.99\,±\,3.35 \\
  & \textbf{AdaptTuner (Ours)} & \textbf{98.86\,±\,0.05} & \textbf{91.21\,±\,0.13} & \textbf{97.47\,±\,0.07} & \textbf{94.27\,±\,0.20} & \textbf{90.90\,±\,0.12} & \textbf{99.43\,±\,0.04} & \textbf{74.79\,±\,0.95} & \textbf{80.10\,±\,0.51} & \textbf{90.00\,±\,0.11} \\
\midrule
\bottomrule
\end{tabular}
\end{table}

==> tables/table_param_efficiency.tex <==
\begin{table}[t]
\centering
\caption{Trainable parameter counts (mean over seeds). Ratio = trainable / total (\%).}
\label{tab:params}
\setlength{\tabcolsep}{5pt}
\footnotesize
\begin{tabular}{l l r r}
\toprule
\textbf{Backbone} & \textbf{Method} & \textbf{Trainable} & \textbf{Ratio (\%)} \\
\midrule
\multirow{3}{*}{DeiT-Ti/16}
  & Head-Only & 18,442 & 0.33 \\
  & Full Fine-Tune & 5,542,858 & 100.00 \\
  & \textbf{AdaptTuner (Ours)} & 94,666 & 1.68 \\
\midrule
\multirow{3}{*}{ViT-S/16}
  & Head-Only & 36,788 & 0.17 \\
  & Full Fine-Tune & 21,702,452 & 100.00 \\
  & \textbf{AdaptTuner (Ours)} & 189,044 & 0.87 \\
\midrule
\multirow{3}{*}{ViT-B/16}
  & Head-Only & 73,482 & 0.09 \\
  & Full Fine-Tune & 85,872,138 & 100.00 \\
  & \textbf{AdaptTuner (Ours)} & 377,802 & 0.44 \\
\midrule
\bottomrule
\end{tabular}
\end{table}
